Quickest Change Detection in Statistically Periodic Processes with Unknown Post-Change Distribution

Algorithms are developed for the quickest detection of a change in statistically periodic processes. These are processes in which the statistical properties are nonstationary but repeat after a fixed time interval. It is assumed that the pre-change law is known to the decision maker but the post-change law is unknown. In this framework, three families of problems are studied: robust quickest change detection, joint quickest change detection and classification, and multislot quickest change detection. In the multislot problem, the exact slot within a period where a change may occur is unknown. Algorithms are proposed for each problem, and either exact optimality or asymptotic optimal in the low false alarm regime is proved for each of them. The developed algorithms are then used for anomaly detection in traffic data and arrhythmia detection and identification in electrocardiogram (ECG) data. The effectiveness of the algorithms is also demonstrated on simulated data.

==> LatexShorts.tex <==
\newtheorem{theorem}{Theorem}[section]
%\newtheorem{proof}{Proof}
\newtheorem{corrly}{Corollary}[theorem]
\newtheorem{prop}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{algorithm}{Algorithm}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{problem}{Problem}[section]


\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Expect}{\mathbb{E}}
\newcommand{\indic}{\mathbb{I}}
\newcommand{\defeq}{\overset{\Delta}{=}}
\newcommand{\hLam}{\tilde{\Lambda}}
\newcommand{\epp}{\epsilon}


\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}


%
\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}
%\DeclareMathOperator{\Pb}{\mathsf{P}}
%\DeclareMathOperator{\Eb}{\mathsf{E}}
\newcommand{\ADD}{{\mathsf{ADD}}}
\newcommand{\CADD}{{\mathsf{CADD}}}
\newcommand{\SADD}{{\mathsf{SADD}}}
\newcommand{\WADD}{{\mathsf{WADD}}}
\newcommand{\FAR}{{\mathsf{FAR}}}
\newcommand{\ARL}{{\mathsf{ARL}}}
\newcommand{\PFA}{\mathsf{PFA}}
\newcommand{\MDD}{{\mathsf{MDD}}}
\newcommand{\ARE}{{\mathsf{ARE}}}
\newcommand{\Var}{{\mathsf{Var}}}
\newcommand{\ANO}{{\mathsf{ANO}}}
\newcommand{\PDC}{{\mathsf{PDC}}}
\newcommand{\PTC}{{\mathsf{PTC}}}
\newcommand{\CPDC}{{\mathsf{CPDC}}}

%
\newcommand{\mc}[1]{\mathcal{#1}} %% use \mc{symb}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Fc}{\mc{F}}
\newcommand{\Pc}{{\mc{P}}}
\newcommand{\Ic}{{\mc{I}}}
\newcommand{\Xc}{{\mc{X}}}
\newcommand{\Cc}{{\mc{C}}}
\newcommand{\Sc}{{\mc{S}}}
\newcommand{\Dd}{{\mc{D}}}

%mathbold
\newcommand{\mbf}[1]{\mathbf{#1}}
%\newcommand{\Pb}{{\mbf{P}}}
%\newcommand{\Eb}{{\mbf{E}}}
\newcommand{\Xb}{{\mbf{X}}}
\newcommand{\Ub}{{\mbf{U}}}
\newcommand{\Zb}{{\mbf{Z}}}

\newcommand{\mb}[1]{\boldsymbol{#1}} %% use \mb{symb}
\newcommand{\Deb}{\mb{\Delta}}
%\newcommand{\class}{\Deb(\ga)}

%mathroman
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\pt}{{\mrm{pt}}}
\newcommand{\Mp}{M_{\pt}}
\newcommand{\J}{{\mrm{J}}}
\newcommand{\D}{{\mrm{D}}}
\newcommand{\I}{{\mrm{I}}}
\newcommand{\tot}{{\mrm{tot}}}


%% mathbb
\newcommand{\mbb}[1]{\mathbb{#1}} %use \mbb{symb}
\def\One{\mathchoice{\rm 1\mskip-4.2mu l}{\rm 1\mskip-4.2mu l}
{\rm 1\mskip-4.6mu l}{\rm 1\mskip-5.2mu l}}
%\newcommand\Ind[1]{{\One_{\{#1\}}}}
\newcommand{\Ib}{\mbb{I}}
\newcommand{\class}{\mbb{C}_\gamma}
\newcommand{\classC}{\mbb{C}}
%
\newcommand{\la}{\lambda}
\newcommand{\De}{\Delta}
\newcommand{\de}{\delta}
\newcommand{\te}{\theta}
\newcommand{\ga}{\gamma}
\newcommand{\si}{\sigma}
\newcommand{\al}{\alpha}
\newcommand{\vae}{\varepsilon}
\newcommand{\hte}{\hat{\te}}
\newcommand{\hde}{\hat{\de}}
%
\newcommand{\xra}{\xrightarrow} %% use \xla{\text{prob}} matches the length of arrow
\newcommand{\Llra}{\Longleftrightarrow}
\newcommand{\Lra}{\Longrightarrow}
\newcommand{\bl}{\bigl}
\newcommand{\br}{\bigr}
\newcommand{\Bl}{\Bigl}
\newcommand{\Br}{\Bigr}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\seq}[1]{\left<#1\right>}
\newcommand{\brc}[1]{\left(#1\right)}
\newcommand{\brcs}[1]{\left[#1\right]}
\newcommand{\vli}{\varliminf}
\newcommand{\vls}{\varlimsup}
\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}

%
\newcommand{\taunc}{\tau_{\scriptscriptstyle \text{MC}}}
\newcommand{\taund}{\tau_{\scriptscriptstyle \text{MD}}}


\newcommand{\taus}{\tau_{\scriptscriptstyle \mathrm{S}}}
\newcommand{\tauc}{\tau_{\scriptscriptstyle \mathrm{C}}}
\newcommand{\tausr}{\tau_{\scriptscriptstyle \mathrm{SR}}}
\newcommand{\tausrp}{\tau_{\scriptscriptstyle \mathrm{SRP}}}
\newcommand{\tausrr}{\tau_{\scriptscriptstyle \mathrm{SR}-r}}
\newcommand{\taug}{\tau_{\scriptscriptstyle \mathrm{G}}}
\newcommand{\taum}{\tau_{\scriptscriptstyle \mathrm{M}}}
\newcommand{\htaug}{\hat{\tau}_{\scriptscriptstyle \mathrm{G}}}
\newcommand{\htaum}{\hat{\tau}_{\scriptscriptstyle \mathrm{M}}}
\newcommand{\taugc}{\tau_{\scriptscriptstyle \mathrm{GC}}}
\newcommand{\taugd}{\tau_{\scriptscriptstyle \mathrm{GD}}}
\newcommand{\taucc}{\tau_{\scriptscriptstyle \mathrm{CC}}}


\newcommand{\taud}{\tau_{\scriptscriptstyle \mathrm{D}}}
\newcommand{\tauw}{\tau_{\scriptscriptstyle \mathrm{W}}}
\newcommand{\tauall}{\tau_{\scriptscriptstyle \mathrm{All}}}
\newcommand{\taudeall}{\tau_{\scriptscriptstyle \mathrm{DE-All}}}
\newcommand{\tauA}{\tau_{\scriptscriptstyle \mathrm{DE-Censor-Sum}}}
\newcommand{\taudist}{\tau_{\scriptscriptstyle \mathrm{DE-Dist}}}
\newcommand{\Psid}{\Psi_{\scriptscriptstyle \mathrm{D}}}
\newcommand{\tauB}{\tau_{\scriptscriptstyle \mathrm{DE-Censor-Max}}}
\newcommand{\taumax}{\tau_{\scriptscriptstyle \mathrm{DE-Censor-Max}}}
\newcommand{\tausum}{\tau_{\scriptscriptstyle \mathrm{DE-Censor-Sum}}}
\newcommand{\taudcm}{\tau_{\scriptscriptstyle \mathrm{DCM}}}
\newcommand{\taudcs}{\tau_{\scriptscriptstyle \mathrm{DCS}}}


%\newcommand{\lambdad}{\lambda_{\scriptscriptstyle \text{D}}}
%\newcommand{\Lambdad}{\Lambda_{\scriptscriptstyle \text{D}}}
\newcommand{\lambdad}{\lambda_{\scriptscriptstyle \mathrm{A}}}
\newcommand{\Lambdad}{\Lambda_{\scriptscriptstyle \mathrm{A}}}


\newcommand{\Psic}{\Psi_{\scriptscriptstyle \mathrm{C}}}
\newcommand{\Psiw}{\Psi_{\scriptscriptstyle \mathrm{W}}}
\newcommand{\Piw}{\Pi_{\scriptscriptstyle \mathrm{W}}}
\newcommand{\Pideall}{\Pi_{\scriptscriptstyle \mathrm{DE-All}}}
\newcommand{\Piall}{\Pi_{\scriptscriptstyle \mathrm{All}}}
\newcommand{\Pif}{\Pi_{\scriptscriptstyle \mathrm{F}}}
\newcommand{\Pimax}{\Pi_{\scriptscriptstyle \mathrm{Max}}}
\newcommand{\Pisum}{\Pi_{\scriptscriptstyle \mathrm{Sum}}}
\newcommand{\Pidcm}{\Pi_{\scriptscriptstyle \mathrm{DCM}}}
\newcommand{\Pidcs}{\Pi_{\scriptscriptstyle \mathrm{DCS}}}


%\newcommand{\Nd}{N_{\scriptscriptstyle \text{D}}}
\newcommand{\Nd}{N_{\scriptscriptstyle \mathrm{A}}}
\newcommand{\lambdaInf}{\lambda_{\scriptscriptstyle \infty}}
\newcommand{\LambdaInf}{\Lambda_{\scriptscriptstyle \infty}}

\newcommand{\Xn}{\{X_n\}}
\newcommand{\Yn}{\{Y_n\}}
\newcommand{\Xnl}{\{X_{n,\ell}\}}
\newcommand{\Xkl}{X_{k, \ell}}
\newcommand{\Ynl}{\{Y_{n, \ell}\}}
\newcommand{\Ykl}{Y_{n, \ell}}

\newcommand{\nuwl}{\nu_{{\scriptscriptstyle \mathrm{W}}, \ell}}
\newcommand{\nucl}{\nu_{{\scriptscriptstyle \mathrm{C}}, \ell}}
\newcommand{\nurl}{\nu_{{\scriptscriptstyle \mathrm{R}}, \ell}}

\newcommand{\tauwl}{\tau_{{\scriptscriptstyle \mathrm{W}}, \ell}}
\newcommand{\taucl}{\tau_{{\scriptscriptstyle \mathrm{C}}, \ell}}
\newcommand{\taurl}{\tau_{{\scriptscriptstyle \mathrm{R}}, \ell}}

\newcommand{\taur}{\tau_{\scriptscriptstyle \mathrm{R}}}

\newenvironment{pfof}[1]{\vspace{1ex}\noindent{\bf Proof of #1}\hspace{0.5em}}
	{\hfill\qed\vspace{1ex}}

\newcommand{\tb}[1]{\textcolor{blue}{#1 (TB)}} %  use \tb{text}

